Graphine: A Dataset for Graph-aware Terminology Definition Generation

Precisely defining the terminology is the first step in scientific communication. Developing neural text generation models for definition generation can circumvent the labor-intensity curation, further accelerating scientific discovery. Unfortunately, the lack of large-scale terminology definition dataset hinders the process toward definition generation. In this paper, we present a large-scale terminology definition dataset Graphine covering 2,010,648 terminology definition pairs, spanning 227 biomedical subdisciplines. Terminologies in each subdiscipline further form a directed acyclic graph, opening up new avenues for developing graph-aware text generation models. We then proposed a novel graph-aware definition generation model Graphex that integrates transformer with graph neural network. Our model outperforms existing text generation models by exploiting the graph structure of terminologies. We further demonstrated how Graphine can be used to evaluate pretrained language models, compare graph representation learning methods and predict sentence granularity. We envision Graphine to be a unique resource for definition generation and many other NLP tasks in biomedicine.

==> newtable.tex <==
\begin{table}[th]
 \begin{center}
  \caption{Table comparing the performance of HYPON with comparison approaches on two COVID-19 ontologies, in terms of AUROC (\%). \textit{hyperbolic}, \textit{graph} and \textit{feature}, represent embedding in hyperbolic space, considering graph structure, and considering entity features, respectively. The {\color{dark_b} best method} in each column is colored in {\color{dark_b} blue} and {\color{light_b}second best} is colored in {\color{light_b}light blue}. Error reduction is defined as the improvement of our AUROC over the AUROC of the best comparison approach. HYPON outperforms all comparison approaches with an average error reduction of 26.35\% under 85\% training percent and  10.4\% under 50\% training percent.}
  \label{table1}
  \resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Dataset}         & \multirow{4}{*}{\rotatebox{90}{\textbf{hyperbolic}}} & \multirow{4}{*}{\rotatebox{90}{\textbf{graph}}} & \multirow{3}{*}{\rotatebox{90}{\textbf{feature}}} & \multicolumn{2}{c}{COVID-19 Ontology} & \multicolumn{2}{c}{IDO-COVID19}  \\

\textbf{Growth rate $\theta$} &                   &                 &                  & \multicolumn{2}{c}{$\theta =11.39$}  & \multicolumn{2}{c}{$\theta =4.02$} \\

\textbf{Nodes}          &                   &                 &                  & \multicolumn{2}{c}{2278}       & \multicolumn{2}{c}{395}      \\\cline{5-8} 
\textbf{Training percent (\%)} &                   &                 &                  & 85        & 50        & 85        & 50       \\ \hline
Poincar\'e              & \ding{51}            & \ding{51}          &            & 76.9      & 71.8      & 61.1      & 57.8     \\
Euclidean             &               &\ding{51}          &            & 73.2     & 72.9      & 52.1     & 50.1     \\
\textit{Feature only}     &               &            & \ding{51}             & 51.7         & 52.5        & 56.8        & 54.5       \\ \hline
GCN                &               & \ding{51}          & \ding{51}          & 74.8      & 63.3      & 58.1     &56.2     \\
GAT                &              & \ding{51}          & \ding{51}          & 73.2      &64.2      & 57.1     & 55.1     \\
SAGE               &               & \ding{51}          &\ding{51}          & 74.0      & 65.3      & 56.8      & 55.2     \\ \hline
HNN                & \ding{51}            &           &\ding{51}           & 76.1      & 70.1      & 60.2      & 53.4     \\
MLP                &              &            & \ding{51}          & 78.1      & 66.9      & 59.1      & 57.8    \\ \hline
OWL2Vec &          & \ding{51}         & \ding{51}           & 74.8      & 72.6      & 65.2     &58.1    \\
Opa2Vec &           & \ding{51}         & \ding{51}           & 76.2     & 74.1      & \cellcolor{light_blue}66.1     &58.6    \\
CANE &            & \ding{51}         & \ding{51}           & 76.8      & 74.9      & 65.8     &59.6     \\ \hline
HGCN               & \ding{51}            & \ding{51}         & \ding{51}           & \cellcolor{light_blue}78.5      & 72.1      & 63.6     &\cellcolor{light_blue}61.1     \\
HGNN               & \ding{51}            & \ding{51}        & \ding{51}           & 76.5      & \cellcolor{light_blue}73.1      &62.8     & 60.1     \\ \hline
Ours               & \ding{51}            & \ding{51}          & \ding{51}          & \cellcolor{new_blue}\textbf{83.3}  & \cellcolor{new_blue}\textbf{76.2}  & \cellcolor{new_blue}\textbf{73.9} & \cellcolor{new_blue}\textbf{64.7} \\ \hline
Error Reduction ($\%$)      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}       & -24.4\%     & -11.5\%      & -28.2\%     & -9.3\%     \\ \bottomrule
\end{tabular}
}

 \end{center}
\end{table}
